Reducing Electricity Demand Charge for Data Centers with Partial Execution

Data centers consume a large amount of energy and incur substantial electricity cost. In this paper, we study the familiar problem of reducing data center energy cost with two new perspectives. First, we find, through an empirical study of contracts from electric utilities powering Google data centers, that demand charge per kW for the maximum power used is a major component of the total cost. Second, many services such as Web search tolerate partial execution of the requests because the response quality is a concave function of processing time. Data from Microsoft Bing search engine confirms this observation. We propose a simple idea of using partial execution to reduce the peak power demand and energy cost of data centers. We systematically study the problem of scheduling partial execution with stringent SLAs on response quality. For a single data center, we derive an optimal algorithm to solve the workload scheduling problem. In the case of multiple geo-distributed data centers, the demand of each data center is controlled by the request routing algorithm, which makes the problem much more involved. We decouple the two aspects, and develop a distributed optimization algorithm to solve the large-scale request routing problem. Trace-driven simulations show that partial execution reduces cost by $3\%--10.5\%$ for one data center, and by $15.5\%$ for geo-distributed data centers together with request routing.

==> Makefile <==
# Makefile for LaTeX document files
# Created by Baochun Li, bli@eecg.toronto.edu, March 30 2001
# Last modified: September 27 2002 

DOCUMENT=main

default: $(DOCUMENT).pdf

$(DOCUMENT).toc: $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

$(DOCUMENT).pdf: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	pdflatex $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

#--------------------------------------------------
# $(DOCUMENT).ps: $(DOCUMENT).dvi
# 	dvips -t letter -Ppdf -G0 -o $@ $<
# 
# $(DOCUMENT).pdf: $(DOCUMENT).ps
# 	cat $(DOCUMENT).ps | ps2pdf - > $(DOCUMENT).pdf 
#-------------------------------------------------- 

all: $(DOCUMENT).pdf

clean:
	rm -rf *.aux $(DOCUMENT).log $(DOCUMENT).toc \
     $(DOCUMENT).bbl $(DOCUMENT).blg $(DOCUMENT).pdf \

